MAR: Masked Autoencoders for Efficient Action Recognition

Standard approaches for video recognition usually operate on the full input videos, which is inefficient due to the widely present spatio-temporal redundancy in videos. Recent progress in masked video modelling, i.e., VideoMAE, has shown the ability of vanilla Vision Transformers (ViT) to complement spatio-temporal contexts given only limited visual contents. Inspired by this, we propose propose Masked Action Recognition (MAR), which reduces the redundant computation by discarding a proportion of patches and operating only on a part of the videos. MAR contains the following two indispensable components: cell running masking and bridging classifier. Specifically, to enable the ViT to perceive the details beyond the visible patches easily, cell running masking is presented to preserve the spatio-temporal correlations in videos, which ensures the patches at the same spatial location can be observed in turn for easy reconstructions. Additionally, we notice that, although the partially observed features can reconstruct semantically explicit invisible patches, they fail to achieve accurate classification. To address this, a bridging classifier is proposed to bridge the semantic gap between the ViT encoded features for reconstruction and the features specialized for classification. Our proposed MAR reduces the computational cost of ViT by 53% and extensive experiments show that MAR consistently outperforms existing ViT models with a notable margin. Especially, we found a ViT-Large trained by MAR outperforms the ViT-Huge trained by a standard training scheme by convincing margins on both Kinetics-400 and Something-Something v2 datasets, while our computation overhead of ViT-Large is only 14.5% of ViT-Huge.

==> contributions.tex <==
Zhiwu Qing:
a. Made a significant intellectual contribution to the implementation of whole experimental system including but not limited to the efficient implementation of ideas, the model construction, the reproduction of the codes and the deployment of the experiments.
b. Contributed to the preparation materials for the methodology part and writing the draft of the full manuscript.



Shiwei Zhang:
a. Made a significant intellectual contribution to the core ideas of the manuscript. Participating in the design of the analytical experiments, optimizing code implementation, and reproducing the results of the related works.
b. Contributed to the preparation materials for the related works, revising the introduction of the article.



Ziyuan Huang:
a. Made a significant intellectual contribution to the analysis of the experiments. Applying the statistical and mathematical techniques to analyze the experimental results, and investigating relevant theoretical explanations.
b. Contributed to the preparation materials for the experiments part, editing the figures and tables in the experiment part of the manuscript.


Xiang Wang:
a. Made a significant intellectual contribution to the investigation of the existing published works and software developments. Participating in the design of experiments, collecting the related pre-trained models and datasets.
b. Contributed to revising the experiments of the manuscript, reviewing the experiments of the manuscript.


Yuehuan Wang:
a. Made a significant intellectual contribution to the visualizations of the experimental results. Participating in the design of the experiments, making an in-depth theoretical analysis of the experimental results, and looking for the theoretical basis.
b. Contributed to revising the methodology of the manuscript.


Yiliang Lv:
a. Made a significant intellectual contribution to the guidance of the detailed experimental designs and experimental optimization. Addressing the demand for computational resources for large model experiments.
b. Contributed to revising the related works of the manuscript. 



Changxin Gao:
a. Made a significant intellectual contribution to the formulation of research goals and aims. Participating in the design of the system, reviewing and editing the figures in the methodology part of the manuscript and analyzing the experimental results;
b. Contributed to the critical review and commentary of the manuscript.


Nong Sang:
a. Made a significant intellectual contribution to the guidance of the theoretical basis of experimental results, and leadership and supervision responsibility for the research activity planning and
execution;
b. Contributed to the preparation materials for the introduction part, critical review and commentary of the full manuscript.


